A novel four-field mixed variational approach to Kirchhoff rods implemented with finite element exterior calculus

A four-field mixed variational principle is proposed for large deformation analysis of Kirchhoff rods with a $C^0$ mixed FE approximations. The core idea behind the approach is to introduce a one-parameter family of points (the centerline) and a separate one-parameter family of orthonormal frames (the Cartan moving frame) that are specified independently. The curvature and torsion of the curve are related to the relative rotation of neighboring frames. The relationship between the frame and the centerline is then enforced at the solution step using a Lagrange multiplier (which plays the role of section force). Well known frames like the Frenet-Serret are defined only using the centerline, which demands higher-order smoothness for the centerline approximation. Decoupling the frame from the position vector of the base curve leads to a description of torsion and curvature that is independent of the position information, thus allowing for simpler interpolations. This approach is then cast in the language of exterior calculus. In this framework, the strain energy may be interpreted as a differential form leading to the natural force-displacement (velocity) pairing. The four-field mixed variational principle we propose has frame, differential forms, and position vector as input arguments. While the position vector is interpolated linearly, the frames are interpolated as piecewise geodesics on the rotation group. Similarly, consistent interpolation schemes are also adopted to obtain finite dimensional approximations for other differential forms aswell. Using these discrete approximations, a discrete mixed variational principle is laid out which is then numerically extremized. The discrete approximation is then applied to benchmark problems, our numerical studies reveal an impressive performance of the proposed method without numerical instabilities or locking.

==> images/deformationMap-1.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'deformationMap.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{340.15748031bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.5)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{./images/deformationMap.pdf}}%
    \put(0.19,0.11){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\bs{\Gamma}(s)$}}}%
    \put(0.71836268,0.11379547){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\bs{\gamma}(s)$}}}%
    \put(0.86870181,0.46124598){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\text{Deformed configuration}$}}}%
    \put(0.12925611,0.44120064){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\text{Reference configuration}$}}}%
    \put(0.1601,0.3844059){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{E}_3$}}}%
    \put(0.25955003,0.31095194){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{E}_1$}}}%
    \put(0.1515286,0.27081629){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{E}_2$}}}%
    \put(0.79297549,0.39442851){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{e}_3$}}}%
    \put(0.90656509,0.33651988){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{e}_1$}}}%
    \put(0.78295288,0.28083878){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\tb{e}_2$}}}%
    \put(0.3449041,0.01113637){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$0$}}}%
    \put(0.51974293,0.01002274){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$L$}}}%
    \put(0.4306531,0.01225001){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$s$}}}%
    \put(0.51456973,0.41892827){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\bs{\chi}$}}}%
  \end{picture}%
\endgroup%


